Coxeter diagrams and the K\"othe's problem

A ring $\Lambda$ is called right K\"othe if every right $\Lambda$-module is a direct sum of cyclic modules. In this paper, we give a characterization of basic hereditary right K\"othe rings in terms of their Coxeter valued quivers. Also we give a characterization of basic right K\"othe rings with radical square zero. Therefore we give a solution of the K\"othe's problem in this cases.

==> DoneTwoElBendy.tex <==
\begin{dynkinDiagram}[ply=4]{D}[1]%
{****.*****.*****}
	\dynkinFold[bend right=90]{1}{13}
	\dynkinFold[bend right=90]{0}{14}
\end{dynkinDiagram}


==> DoneTwoElStraight.tex <==
\begin{dynkinDiagram}[ply=4]{D}[1]%
{****.*****.*****}
	\dynkinFold{0}{1}
	\dynkinFold{1}{13}
	\dynkinFold{13}{14}
\end{dynkinDiagram}


==> EulerProducts.tex <==
\tikzset{/Dynkin diagram,ordering=Dynkin,label macro/.code={\alpha_{#1}}}
\newcounter{EPNo}
\setcounter{EPNo}{0}
\NewDocumentCommand\EP{smmmm}%
{%
\stepcounter{EPNo}\roman{EPNo}. &
\def\eL{.6cm}
\IfStrEqCase{#2}%
{%
{D}{\gdef\eL{1cm}}%
{E}{\gdef\eL{.75cm}}%
{F}{\gdef\eL{.35cm}}%
{G}{\gdef\eL{.35cm}}%
}%
\tikzset{/Dynkin diagram,edge length=\eL}
\IfBooleanTF{#1}%
{\dynkin[backwards,labels*={#4},labels={#5}]{#2}{#3}}
{\dynkin[labels*={#4},labels={#5}]{#2}{#3}}
\\
}%
\begin{longtable}{MM}
\caption{Dynkin diagrams from Euler products \cite{Langlands:1967}}\\
\endfirsthead
\caption{\dots continued}\\
\endhead
\multicolumn{2}{c}{continued \dots}\\
\endfoot
\endlastfoot
\EP{A}{***.**}{1,1,1,1,1}{,1,2,n-1,n}
\EP{A}{***.**}{1,1,1,1,1}{1,2,n-1,n}
\EP{A}{**.***.*}{1,1,1,1,1,1}{1,2,m-1,,m,n}
\EP{B}{**.***}{2,2,2,2,1}{1,2,n-1,n}
\EP*{B}{***.**}{2,2,2,2,1}{n,n-1,2,1,}
\EP{C}{**.***}{1,1,1,1,2}{1,2,n-1,}
\EP*{C}{***.**}{1,1,1,1,2}{n,n-1,2,1,}
\EP{D}{**.****}{1,1,1,1,1,1}{1,2,n-2,n-1,n}
\EP{D}{**.****}{1,1,1,1,1,1}{1,2,n-2,n-1,n}
\EP{E}{6}{1,1,1,1,1,1}{1,...,5}
\EP*{E}{7}{1,1,1,1,1,1,1}{6,...,1}
\EP{E}{7}{1,1,1,1,1,1,1}{1,...,6}
\EP*{E}{8}{1,1,1,1,1,1,1,1}{7,...,1}
\EP{E}{8}{1,1,1,1,1,1,1,1}{1,...,7}
\EP{G}{2}{1,3}{,1}
\EP{G}{2}{1,3}{1}
\EP{B}{**.*.**}{2,2,2,2,1}{,1,2,n-1,n}
\EP{F}{4}{1,1,2,2}{,3,2,1}
\EP{C}{3}{1,1,2}{,2,1}
\EP{C}{**.***}{1,1,1,1,2}{,1,n-2,n-1,n}
\EP*{B}{3}{2,2,1}{1,2}
\EP{F}{4}{1,1,2,2}{1,2,3}
\EP{D}{**.****}{1,1,1,1,1,1}{1,2,n-2,n-2,n,n}
\EP{E}{6}{1,1,1,1,1,1}{1,2,3,4,,5}
\EP{E}{6}{1,1,1,1,1,1}{1,2,3,5,,4}
\EP*{E}{7}{1,1,1,1,1,1,1}{,5,...,1,6}
\EP*{E}{7}{1,1,1,1,1,1,1}{,6,4,3,2,1,5}
\EP*{E}{8}{1,1,1,1,1,1,1,1}{,6,...,1,7}
\EP*{E}{8}{1,1,1,1,1,1,1,1}{,7,5,4,3,2,1,6}
\EP*{E}{7}{1,1,1,1,1,1,1}{5,...,1,,6}
\EP*{E}{7}{1,1,1,1,1,1,1}{1,...,5,,6}
\EP*{E}{8}{1,1,1,1,1,1,1,1}{6,...,1,,7}
\end{longtable}


==> borovoi.tex <==
\tikzset{big arrow/.style={
	-Stealth,line cap=round,line width=1mm,
	shorten <=1mm,shorten >=1mm}}
\newcommand\catholic[2]{\draw[big arrow,green!25!white] 
(root #1) to (root #2);}
\newcommand\protestant[2]{
\begin{scope}[transparency group, opacity=.25]
\draw[big arrow,orange] (root #1) to (root #2);
\end{scope}}
\begin{dynkinDiagram}[edge length=1.2cm,
indefinite edge/.style={thick,loosely dotted},
labels*={0,1,2,3,\ell-3,\ell-2,\ell-1,\ell}]{D}[1]{}
\catholic{0}{6}\catholic{1}{7}
\protestant{7}{0}\protestant{6}{1}
\end{dynkinDiagram}


==> d44.tex <==
\tikzset{/Dynkin diagram,edge length=1cm,fold radius=1cm}
\tikzset{/Dynkin diagram,label macro/.code={\alpha_{#1}},label macro*/.code={\beta_{#1}}}
\({}^1 D_4\) 4-ply tied straight:
\begin{dynkinDiagram}[ply=4]{D}[1]%
{****.*****.*****}
 \dynkinFold{0}{1}
 \dynkinFold{1}{13}
 \dynkinFold{13}{14}
\dynkinLabelRoots{0,...,14}
\dynkinLabelRoots*{0,...,14}
\end{dynkinDiagram}
\({}^1 D_4\) 4-ply tied bending:
\begin{dynkinDiagram}[ply=4]{D}[1]%
{****.*****.*****}
	\dynkinFold{1}{13}
	\dynkinFold[bend right=65]{0}{14}
\dynkinLabelRoots{0,...,14}
\dynkinLabelRoots*{0,...,14}
\end{dynkinDiagram}


==> hermitian-symmetric-spaces.tex <==
\NewDocumentCommand\HSS{mommm}
{#1&\IfNoValueTF{#2}{\dynkin{#3}{#4}}{\dynkin[parabolic=#2]{#3}{#4}}&#5\\}
\renewcommand*{\arraystretch}{1.5}
\begin{longtable}
{>{\columncolor[gray]{.9}}>$l<$>{\columncolor[gray]{.9}}>$l<$>{\columncolor[gray]{.9}}l}
\caption{The Hermitian symmetric spaces}\endfirsthead
\caption{\dots continued}\\ \endhead
\caption{continued \dots}\\ \endfoot
\endlastfoot
\HSS{A_n}{A}{**.*x*.**}{Grassmannian of $k$-planes in $\C{n+1}$}
\HSS{B_n}[1]{B}{}{$(2n-1)$-dimensional hyperquadric, i.e. the variety of null lines in $\C{2n+1}$}
\HSS{C_n}[16]{C}{}{space of Lagrangian $n$-planes in $\C{2n}$}
\HSS{D_n}[1]{D}{}{$(2n-2)$-dimensional hyperquadric, i.e. the variety of null lines in $\C{2n}$}
\HSS{D_n}[32]{D}{}{one component of the variety of maximal dimension null subspaces of $\C{2n}$}
\HSS{D_n}[16]{D}{}{the other component}
\HSS{E_6}[1]{E}{6}{complexified octave projective plane}
\HSS{E_6}[32]{E}{6}{its dual plane}
\HSS{E_7}[64]{E}{7}{the space of null octave 3-planes in octave 6-space}
\end{longtable}


==> simple-lie-algebras.tex <==
\NewDocumentEnvironment{bunch}{}%
{\renewcommand*{\arraystretch}{1}\begin{array}{@{}ll@{}}\\ \midrule}{\\ \midrule\end{array}}
\small
\NewDocumentCommand\nct{mm}{\newcolumntype{#1}{>{\columncolor[gray]{.9}}>{$}m{#2cm}<{$}}}
\nct{G}{.3}\nct{D}{2.1}\nct{W}{3}\nct{R}{3.7}\nct{S}{3}
\NewDocumentCommand\LieG{}{\mathfrak{g}}
\NewDocumentCommand\W{om}{\ensuremath{\mathbb{Z}^{#2}\IfValueT{#1}{/\left<#1\right>}}}
\renewcommand*{\arraystretch}{1.5}
\NewDocumentCommand\quo{}{\text{quotient of } E_8}
\begin{longtable}{@{}GDWRS@{}}
\LieG&\text{Diagram}&\text{Weights}&\text{Roots}&\text{Simple roots}\\ \midrule\endfirsthead
\LieG&\text{Diagram}&\text{Weights}&\text{Roots}&\text{Simple roots}\\ \midrule\endhead
A_n&\dynkin{A}{}&\frac{1}{r+1}\W[\sum e_j]{n+1}&e_i-e_j&e_i-e_{i+1}\\
B_n&\dynkin{B}{}&\frac{1}{2}\W{n}& \pm e_i, \pm e_i \pm e_j, i\ne j&e_i-e_{i+1}, e_n\\
C_n&\dynkin{C}{}&\W{n}& \pm 2 e_i, \pm e_i \pm e_j, i\ne j&e_i-e_{i+1}, 2e_n\\
D_n&\dynkin{D}{}&\frac{1}{2}\W{n}& \pm e_i \pm e_j, i\ne j &
\begin{bunch}e_i-e_{i+1},&i\le n-1\\e_{n-1}+e_n\end{bunch}\\
E_8&\dynkin{E}{8}&\frac{1}{2}\W{8}&
\begin{bunch}\pm2e_i\pm2e_j,&i\ne j,\\ \sum_i(-1)^{m_i}e_i,&\sum m_i \text{ even}\end{bunch}&
\begin{bunch}
2e_1-2e_2,\\2e_2-2e_3,\\2e_3-2e_4,\\2e_4-2e_5,\\2e_5-2e_6,\\2e_6+2e_7,\\
-\sum e_j,\\2e_6-2e_7
\end{bunch}\\
E_7&\dynkin{E}{7}&\frac{1}{2}\W[e_1-e_2]{8}&\quo&\quo\\
E_6&\dynkin{E}{6}&\frac{1}{3}\W[e_1-e_2,e_2-e_3]{8}&\quo&\quo\\
F_4& \dynkin{F}{4}&\W{4}&
\begin{bunch}\pm 2e_i,\\ \pm 2e_i \pm 2e_j, \quad i \ne j,\\ \pm e_1 \pm e_2 \pm e_3 \pm e_4
\end{bunch}&
\begin{bunch}2e_2-2e_3,\\2e_3-2e_4,\\2e_4,\\e_1-e_2-e_3-e_4\end{bunch}\\
G_2&\dynkin{G}{2}&\W[\sum e_j]{3}&
\begin{bunch}
\pm(1,-1,0),\\ \pm(-1,0,1),\\ \pm(0,-1,1),\\ \pm(2,-1,-1),\\ \pm(1,-2,1),\\ \pm(-1,-1,2)
\end{bunch}&
\begin{bunch}(-1,0,1),\\(2,-1,-1)\end{bunch}
\end{longtable}

